Monocular Dynamic Gaussian Splatting: Fast, Brittle, and Scene Complexity Rules

Gaussian splatting methods are emerging as a popular approach for converting multi-view image data into scene representations that allow view synthesis. In particular, there is interest in enabling view synthesis for dynamic scenes using only monocular input data -- an ill-posed and challenging problem. The fast pace of work in this area has produced multiple simultaneous papers that claim to work best, which cannot all be true. In this work, we organize, benchmark, and analyze many Gaussian-splatting-based methods, providing apples-to-apples comparisons that prior works have lacked. We use multiple existing datasets and a new instructive synthetic dataset designed to isolate factors that affect reconstruction quality. We systematically categorize Gaussian splatting methods into specific motion representation types and quantify how their differences impact performance. Empirically, we find that their rank order is well-defined in synthetic data, but the complexity of real-world data currently overwhelms the differences. Furthermore, the fast rendering speed of all Gaussian-based methods comes at the cost of brittleness in optimization. We summarize our experiments into a list of findings that can help to further progress in this lively problem setting.

==> tex/figures/fig_static_gs.tex <==
\begin{wrapfigure}[9]{r}{4cm}
    \vspace{-0.7cm}
    \centering
    \setlength{\fboxsep}{0pt}
    \label{fig:static_gs}
    \begin{minipage}{0.12\textwidth}
        \includegraphics[width=\textwidth]{images/static_gs/gt.png} 
    \end{minipage}%
    \hspace{0.002\textwidth}
    \begin{minipage}{0.12\textwidth}
        \includegraphics[width=\textwidth]{images/static_gs/rendered.png}
    \end{minipage}%
    \caption{(Left) Train image. (Right) Static 3DGS rendering given inaccurate poses.}
    \label{fig:static_gs_bg}
\end{wrapfigure}

\iffalse
\begin{wrapfigure}[8]{r}{4cm}
    \vspace{-0.7cm}
    \centering
    \setlength{\fboxsep}{0pt}
    \label{fig:static_gs}
    \begin{minipage}{0.12\textwidth}
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{images/static_gs/gt.png}};
            % Define the rectangle for the zoom-in
            \begin{scope}[x={(image.south east)},y={(image.north west)}]
                % Draw the rectangle
                \draw[red,thick] (0.3,0.3) rectangle (0.7,0.7); % Adjust the coordinates as needed
                % Add the zoomed-in image
                \node[anchor=south west,inner sep=0] at (1.2,-0.2) {\includegraphics[width=0.6\textwidth,trim=0.3\width 0.3\height 0.3\width 0.3\height,clip]{images/static_gs/gt.png}};
            \end{scope}
        \end{tikzpicture}
    \end{minipage}%
    \hspace{0.002\textwidth}
    \begin{minipage}{0.12\textwidth}
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{images/static_gs/rendered.png}};
            % Define the rectangle for the zoom-in
            \begin{scope}[x={(image.south east)},y={(image.north west)}]
                % Draw the rectangle
                \draw[red,thick] (0.3,0.3) rectangle (0.7,0.7); % Adjust the coordinates as needed
                % Add the zoomed-in image
                \node[anchor=south west,inner sep=0] at (1.2,-0.2) {\includegraphics[width=0.6\textwidth,trim=0.3\width 0.3\height 0.3\width 0.3\height,clip]{images/static_gs/rendered.png}};
            \end{scope}
        \end{tikzpicture}
    \end{minipage}%
    \caption{TODO}
    \label{fig:static_gs_bg}
\end{wrapfigure}
\fi
